Formalization of Automated Trading Systems in a Concurrent Linear Framework

We present a declarative and modular specification of an automated trading system (ATS) in the concurrent linear framework CLF. We implemented it in Celf, a CLF type checker which also supports executing CLF specifications. We outline the verification of two representative properties of trading systems using generative grammars, an approach to reasoning about CLF specifications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{T. Ehrhard, M. Fern\'andez, V. de Paiva, L. Tortora de Falco (Eds.):\\ Linearity-TLLA 2018\\
EPTCS 292, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.292.1}{10.4204/EPTCS.292.1}}
\pdfoutput=1

